Equality, Quasi-Implicit Products, and Large Eliminations

This paper presents a type theory with a form of equality reflection: provable equalities can be used to coerce the type of a term. Coercions and other annotations, including implicit arguments, are dropped during reduction of terms. We develop the metatheory for an undecidable version of the system with unannotated terms. We then devise a decidable system with annotated terms, justified in terms of the unannotated system. Finally, we show how the approach can be extended to account for large eliminations, using what we call quasi-implicit products.

==> eptcsdata.tex <==
\providecommand{\firstpage}{90}
\providecommand{\publicationstatus}{E. Pimentel, B. Venneri and J. Wells (Eds.): Workshop on\\
Intersection Types and Related Systems 2010 (ITRS 2010).\\
EPTCS 45, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.45.7}{10.4204/EPTCS.45.7}}

